AnnotateThis: Analyzing a human-LLM system for annotating social media data with the concept of climate change mitigation pessimism

Large language models (LLMs) are increasingly being integrated into research workflows. However, LLMs have been shown to struggle with difficult and nuanced concepts such as those found in computational social science (CSS) research. Within the CSS community, there has been a call for new systems to be developed which center humans in LLM-supported scientific workflows. We develop AnnotateThis, a human-centered system for inspecting and improving LLM annotations, a process we refer to as LLM grounding for a target concept. AnnotateThis is developed with both computational and social scientists to reflect existing workflows for data annotation. It includes a range of information features for users to interrogate the quality and reliability of LLM annotations. We evaluate our system in two settings. In the first, we assume a researcher may not have access to ground truth data and that users of AnnotateThis have limited prior knowledge of the concept they would like an LLM to annotate. That is, they may be conducting concept specification and LLM grounding simultaneously. In the second setting, we assume access to ground truth labels and that the concept is specified for a given annotation task; here, the task of LLM grounding is more straightforward. We find that in both settings users can improve the quality of LLM annotations with AnnotateThis and that their final annotations far surpass those created without human intervention. For example, when we evaluate with ground truth labels, we see an absolute improvement of 0.15 in F-Measure and 0.23 in accuracy over a fully automated state-of-the-art method for prompt refinement.

==> AnonymousSubmission/LaTeX/big_table.tex <==
% updated big table with study 1 and 2 combined

\begin{table*}[t]
\small
\caption{To answer our research questions we compare the performance LLM outputs when produced with different input prompts. 
For each set of outputs, we extract the labels and compare these to a set of ground truth expert labels. 
We bold all differences which are statistically significant.
}

\label{tab:prompt_performance24}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccc}
\toprule
\multicolumn{6}{c}{Baseline Metrics}\\
 & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F-Measure} & \textbf{Average  Length of Instructions}\\
\midrule
 Participants & $0.637_{0.029}$ & $0.160_{0.027}$ & $0.567_{0.065}$ & $0.232_{0.033}$ & -\\
First prompts & $0.415_{0.006}$ & $0.156_{0.008}$ & $0.911_{0.024}$ & $0.256_{0.011}$ & 309.2\\ 
 Selected prompts & $0.578_{0.001}$ & $0.246_{0.008}$ & $0.922_{0.022}$ & $0.362_{0.008}$ & 737.8\\
 \midrule
\multicolumn{6}{c}{RQ1: Can participants use
\ourmethode{} to improve their instructions to LLMs?}\\
\multicolumn{6}{c}{$\Delta=$ $\big($performance of selected prompt$\big)$ $-$ $\big($performance of first prompt$\big)$}\\
\midrule
  & \textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \textbf{$\Delta$ Avg Prompt Length}\\
% \sone{} & \textbf{0.137} & \textbf{0.091} & 0.037 & \textbf{0.106} & 395.6\\
% \stwo{} & \textbf{0.185} & \textbf{0.090} & -0.010 & \textbf{0.108} & 461.6\\
& \textbf{0.163} & \textbf{0.090} & 0.011 & \textbf{0.106} & 428.6\\
\midrule
\multicolumn{6}{c}{RQ2: When equipped with instructions from \ourmethode{}{} how do LLMs compare with \subs{}?}\\
\multicolumn{6}{c}{$\Delta=$ $\big($performance of LLM with a prompt$\big)$ $-$ $\big($performance of labels produced by participant$\big)$}\\
\midrule
% First prompts  & \textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \\
% \sone& \textbf{-0.145}&-0.044&0.197&-0.035\\
% \stwo& \textbf{-0.284}&0.028& \textbf{0.464}&0.073\\
% Selected prompts  & \textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \\
% \sone&-.008&.047&.234&.071&\\
% \stwo& \textbf{-.099}&\textbf{.118}&\textbf{.454}&\textbf{.181}&\\

  & \textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \\
First prompts & \textbf{-0.222}&-0.004&\textbf{0.344}&-0.024\\
Selected prompts & -.058&\textbf{.086}&\textbf{.356}&\textbf{.131}&\\

\midrule
%\multicolumn{6}{c}{RQ3: Will \ourmethode{} produce  LLM outputs with more alignment
%with experts than \ourmethod{}?}\\
% \multicolumn{6}{c}{$\Delta=$ $\big($performance of  selected prompt in \stwo{}$\big)$ $-$ $\big($performance of selected prompt in \sone{}$\big)$}\\
%\midrule
% &\textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \textbf{$\Delta$ Avg Prompt Length}\\
% Both studies&\textbf{.117}&   \textbf{.058}&.038&\textbf{.082} & 211.0\\
% \midrule

\multicolumn{6}{c}{RQ3: How does \ourmethod{} compare with a state-of-the-art automated method?}\\
 \multicolumn{6}{c}{$\Delta=$ $\big($performance of selected prompt$\big)$ $-$ $\big($performance of APE$\big)$}\\
\midrule
&\textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \textbf{$\Delta$ Avg Prompt Length}\\
% \sone & \textbf{0.171} & \textbf{0.067} & -0.087 & \textbf{0.069} & 300.0 \\
% \stwo & \textbf{0.234} & \textbf{0.123} & -0.011 & \textbf{0.147} & 453.0\\
& \textbf{0.206} & \textbf{0.098} & -0.044 & \textbf{0.111} & 376.5 \\
\midrule
\multicolumn{6}{c}{RQ5: Will \ourmethode{} produce  LLM outputs with more alignment
with experts than \ourmethod{}?}\\
 \multicolumn{6}{c}{$\Delta=$ $\big($performance of  selected prompt in \stwo{}$\big)$ $-$ $\big($performance of selected prompt in \sone{}$\big)$}\\
\midrule
 &\textbf{$\Delta$Acc} & \textbf{$\Delta$Prec} & \textbf{$\Delta$Recall} & \textbf{$\Delta$F-Measure} & \textbf{$\Delta$ Avg Prompt Length}\\
 s&\textbf{.117}&   \textbf{.058}&.038&\textbf{.082} & 211.0\\
\bottomrule
\end{tabular*}
\end{table*}

==> AnonymousSubmission/LaTeX/checklist.tex <==
\section{Paper Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    % \answerTODO{Answer}
    \answerYes{Yes. We study how domain-relevant and generally non-technical annotators refine LLM prompts for a subjective social science concept. We use public TikTok videos collected via the TikTok Research API and conduct an IRB exempted human subjects study with compensated participants.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, see Empirical Evaluation.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, see Social Media Data Collection and Participant Background in the Appendix.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see Discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, see Discussion.}
      \item Did you discuss any potential misuse of your work?
    \answerYes{At this point we are not releasing a system into the wild. We did discuss the potential misuse of the system at that point, however it is premature given this submission.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{We worked with IRB to ensure that there was no negative consequences for the study participants and included warnings before the videos which were viewed in the studies.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    % \answerTODO{Answer}
    \answerNA{NA. We do not present theoretical results.}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA. (Not applicable as “theoretical results”. Our work is empirical, and we discuss alternative interpretations in discussion.)}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Empirical Evaluation, Table~\ref{tab:sone_performance_full}, Table~\ref{tab:raw_bigtable}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, see Empirical Evaluation, Table~\ref{tab:sone_performance_full}, Table~\ref{tab:raw_bigtable}.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, reported standard error over mean in Table~\ref{tab:sone_performance_full}, Table~\ref{tab:raw_bigtable}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, see Implementation details.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, see Empirical Evaluation.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerNA{NA - our design is such that this is a design for end users of the system.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, the models are assets which we cite.}
  \item Did you mention the license of the assets?
    \answerNA{NA}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNo{We are not permitted to share the raw posts from TikTok which we collect.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes, see Study Statistics in Empirical Evaluation.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{NA, we are not sharing (as we are not permitted to) any data with PII or offensive content.}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
% (see \citet{fair})?
\answerNA{NA}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerYes{Yes. See System Prompt, Tasks, Screenshots of Information Features on Statistics Page, Additional System Screenshots in the Appendix.}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerYes{Yes. We report that the studies were exempt with an institutional IRB and participants completed consent procedures. We included in the consent form specifically ``This study poses no more than minimal risk. You may skip any question or withdraw from the study at any time. Some TikTok content may reference climate-related fear or anxiety; if you find any material upsetting, you are welcome to discontinue at any point.''}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{Yes, see Study Statistics in Empirical Evaluation.}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerYes{Yes, see Data Storage}
\end{enumerate}

\end{enumerate}

==> AnonymousSubmission/LaTeX/empirical.tex <==
\label{sec:empdesign}
%We designed two studies in order to determine the ability of our system to assist RAs in instructing LLMs to annotate social science data.
Our first question is whether our system is successful. That is, we ask
\textbf{RQ1:} Can \subs{} use \ourmethode{} to improve their instructions to LLMs?
By collecting a series of instructions for each participant we can observe whether \subs{} improve these over time.

However, it is not sufficient that \subs{}
write better instructions over time, the final instructions they produce should lead to LLM annotations of a sufficient quality so that LLMs can be used as annotators rather than \subs. That is, \textbf{RQ2:}  When equipped with instructions from \ourmethode{} how do LLMs compare with \subs{}? 


Additionally, we propose that our method will be more successful than fully automated methods which may fail on the task of detecting subjective concepts. Thus we ask, \textbf{RQ3:} How does \ourmethode{} compare with a state-of-the-art automated method?
As we consider a range of information features, we also ask \textbf{RQ4:} Which information features do \subs{} use and do they find the system usable overall?

Finally, an important component of our system is the expert guidance we include. 
As this guidance comes at an increased labor cost from social scientists, it is critical to evaluate whether it leads to better outcomes. We thus compare our method to a baseline version, 
\ourmethod, which has all of the same features as \ourmethode, except for the expert components. Then we ask, 
\textbf{RQ5:} Will \ourmethode{} produce LLM outputs with more alignment with experts than \ourmethod?


To answer these questions we conducted two studies with students enrolled in graduate programs in a program of study on sustainability and environmental science \footnote{One method of recruitment was through physical posters placed in the departmental building, 3 non-student participants out of 60 enrolled in the study in this way and they were staff and faculty in the program on sustainability and environmental science.}.
In both cases the sessions ran for no more than 2 hours and participants received a \$50 virtual credit card. 
Both studies were deemed exempt by an institutional IRB. 
In total, \textbf{60} \subs{} participated across the two studies. 

Participants followed a structured six-step workflow (full details in Appendix~\nameref{app:tasks}): 
\begin{itemize}
    \item Consent form and study introduction.
    \item Short training quiz on 6 practice videos (\stwo{} only).
    \item Label 10 TikTok videos for climate change mitigation pessimism.
    \item Iterate with \textsc{AnnotateThis}: write instructions, view LLM predictions and info features, revise instructions.
    \item Re-annotate the same 10 videos.
    \item Complete a brief post-task survey.
\end{itemize}



\subsection{Study Statistics}
After each study we asked \subs{} to fill out a survey. This included questions about their technical expertise (additional responses to this survey can be found in Appendix~\nameref{app:participants}). We found that 55 out of 60 \subs{} reported that they had no prior experience training LLMs to analyze text data. Thus, for the majority of the \subs{} \ourmethode{} was their first exposure to using LLMs to annotate data. 

In the first study, \sone, 27 \subs{} participated. In \sone, 
participants used all information features besides \elabel{}. They also were not provided with the additional training quiz denoted as \equiz{}. 
In the second study, \stwo,
participants used the full version of \ourmethode, complete with the \equiz{} and \elabel{} components. 



\commentout{
\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{0.95}
  \caption{Study conditions and setup.}
  \label{tab:study-setup}
  \begin{tabular}{p{0.36\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    & Study 1 (Base) & Study 2 (Expert) \\
    \midrule
    Interface                    & \ourmethod       & \ourmethode \\
    Target concept               & CCMP             & CCMP \\
    Alias                        & Climate pessimism & CCMP \\
    Definition                   & See \defnref{def1} & See \defnref{def1} \\
    Training quiz                & No               & Yes \\
    Expert label given for LLM output & No               & Yes \\
    \bottomrule
  \end{tabular}
  \label{tab:studycomp}
\end{table}
}



% \begin{center}
% \begin{myboxf}[colback = white, fontupper=\color{black}]{}
% \begin{minipage}[t]{0.5\textwidth}
% Study 1
% \begin{itemize}
% \item 27 \subs 
% \item Held in  a computer lab in Spring 2025
% \item Used \ourmethod{}
% \end{itemize}
% \end{minipage}
% \begin{minipage}[t]{0.5\textwidth}
% Study 2
% \begin{itemize}
% \item 33 \subs{}
% \item Held over zoom in Summer 2025
% \item Used \ourmethode{}
% \end{itemize}
% \end{minipage}
% \end{myboxf}
% \end{center}


\commentout{
\begin{center}
\begin{myboxf}[colback=white, fontupper=\color{black}]{}%
\begin{minipage}[t]{0.48\linewidth}\raggedright
\textbf{Expert scaffolding}\vspace{2pt}
\begin{itemize}
  \setlength{\itemsep}{2pt}
 % \vspace{-2mm}
  \item 33 \subs{}
  \item Held over Zoom

\end{itemize}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}\raggedright
\textbf{Baseline}\vspace{2pt}
\begin{itemize}
  \setlength{\itemsep}{2pt}
  \setlength{\parsep}{0pt}
  \setlength{\parskip}{0pt}
  \item 27 \subs
  \item Held in a computer lab

\end{itemize}
\end{minipage}
\end{myboxf}
\end{center}
}

\commentout{
The second study was held online as it occurred during the summer when most students were off campus. 
To ensure that the studies were as similar as possible we asked all \subs{} in the virtual sessions to share their screens periodically and to keep their cameras on. 
They were also encouraged to ask questions in chat, to mimic the in-person setting where \subs{} asked the study manager questions.
In both studies  \subs{} asked questions frequently, either by calling over the study manager, or via the chat. }




\subsection{TikTok Dataset on Climate Change Mitigation Pessimism}
We constructed a dataset of TikTok videos relevant to climate change mitigation pessimism through a two-stage scraping and refinement process. The team initially curated a hierarchical list of climate-related terms, including umbrella concepts such as \textit{climate change}, \textit{extreme weather}, and \textit{biodiversity loss}, and more specific terms under each umbrella e.g. \textit{carbon}, \textit{global warming}, and \textit{greenhouse gases} would be specific terms under \textit{climate change}. Using these terms, we collected 21{,}771 TikTok videos using the TikTok Research API  and conducted an exploratory analysis of frequent keywords, n-grams, and keyword co-occurrence patterns. We also sampled representative videos for each keyword to aid expert refinement of the term list.

This process was repeated in a second round with 20{,}435 additional videos based on the revised term set. The final keyword list was selected after reviewing the initial set of videos. 
That is, the team then met together and analyzed the videos. In particular, we discussed how many videos were surfaced for each key term and whether these videos were actually relevant to climate change. This process results in the following set of refined key words: 

\textit{climate change, global warming, ecosystem, greenhouse, climateaction, extreme weather, forestfire, biodiversity loss,  conservation, biodiversity, habitat, environmental degradation, sealevel, sustainability and energy, greenwashing, zero waste, net zero, geoengineering, carbon capture, climate justice}
(Variations in blank space and capitalized letters are added to the key words to ensure we capture a wider range of relevant videos. Detailed keyword selection process is included in the appendix section~\nameref{app:keywords}.)

Using this list, we collected a total of 62{,}513 TikTok videos published between January 1, 2024 and December 31, 2024.
To ensure content relevance, a random subset of 1{,}000 videos was annotated using GPT-4o-mini to determine the presence of three key climate-related themes: (1) effects or harms of climate change, (2) actions to mitigate climate change, and (3) scientific facts about climate change.


From this pseudo-labeled set, 10 videos were selected for manual annotation in the study, and an additional 50 were used for interface testing in \sone.
In \stwo, the interface was tested with 20 videos, as we observed in \sone{} that \subs{} typically viewed 20 videos in a session.


==> AnonymousSubmission/LaTeX/evaluation.tex <==
\section{Climate change mitigation pessimism}
Climate change mitigation pessimism was selected as the focus of this study for several reasons. First, it reflects a growing concern among climate researchers and communicators \citep{davidson2023}.
% \todo{Please add Ariel, Derek\citep{}}. 
Additionally, climate change mitigation pessimism aligns with the academic and personal interests of a broad participant pool. 
We are especially interested in understanding the experiences of non-technical users, and it is important to find a concept of relevance to a wide group of sustainability researchers.
%\gs{next sentence a little akward} 
%This makes it especially suitable for recruiting  graduate students and faculty in sustainability or environmental justice, who may have limited exposure to LLMs but bring relevant interpretive expertise to the task.

Second, the concept presents methodological challenges that make it particularly well-suited for evaluating information-supported annotation workflows for social media data. Climate change mitigation pessimism is subjective, emotionally engaged, and often embedded in subtle language or tone. It may be expressed implicitly — through sarcasm, humor, or despair — rather than through clear propositional statements. 
This makes it difficult to annotate using rule-based heuristics or simple keyword matching. Because interpretations of pessimism can vary across disciplinary backgrounds and personal experiences, the annotation task involves active sensemaking and specification \citep{pirolli2005, dork2011}.



We define climate change mitigation pessimism  as expressions of the belief that humans cannot (or will not) meaningfully reduce the causes or impacts of climate change. The tone is typically hopeless or resigned and may imply giving up on mitigation efforts. Social media users may express this belief in posts about the failure of government to take meaningful action against climate change, or in statements such as ``it is too late'' to do anything about this problem. We operationalize this as shown in \defnref{def1}.
%The operationalization of this concept is shown in \defnref{def} in the same phrasing that it was shown to \subs. 

\begin{definition}[\textbf{Climate Change Mitigation Pessimism}]
 Pessimism with regard to climate change mitigation (the ability to take action to reduce the event
of and effects of climate change). \label{def1}
\end{definition}



==> AnonymousSubmission/LaTeX/intro.tex <==


%Mitigating the negative consequences of climate change will require novel policies. 
%Yet, the success of such policies can be influenced by public attitudes. 

 Social media data serves as a key source for insights into public attitudes about climate change
\citep{galdeman2025mapping,pearce2019social,treen2022discussion,hautea2021showing}. 
Given the overwhelming amount of negative political content on such platforms, users may come to feel overwhelmed, anxious, and fatigued with news and politics,  leading to cynicism and lower levels of political efficacy \citep{lane2025worn,hasell2025social,song2021social}.
One result may be 
that the public will become increasingly convinced that actions to mitigate the consequences of climate change are futile. 
This prompts the question, to what extent does the  public express pessimism  on social media
about humanity's ability to mitigate the negative consequences of climate change?
We refer to this attitude as \textbf{\climate}. 


Typically, to answer this question, a social scientist might begin by training research assistants (RAs), usually students in an expert's core discipline, to annotate (code/label) social media data for the concept of \climate.  
This practice of training RAs is advantageous as it reduces expert time and costs for labor-intensive annotation processes. 
It also transfers knowledge to novices in the field, who learn both from expert instruction and from exposure to the data itself. RAs can also inform experts, leading to broader and more inclusive conceptualizations. 

We develop a system (\ourmethode) which leverages the existing benefits of this practice of training RAs for data annotation, while improving scalability over existing computational methods by utilizing large language models (LLMs). 
With \ourmethode{}, rather than performing annotation, 
RAs can instead 
design instructions for LLMs to code data. If successful, this approach would allow for far larger amounts of data to be coded than is currently possible through RA labor alone. Moreover, this approach would provide RAs in the social sciences both with first-hand exposure to the primary data used in analysis 
\textit{and} with technical systems which may be useful throughout their  careers. 

Our approach aligns with other Human-Centered approaches for utilizing LLMs in data annotation \citep{shin2024understanding,li2023coannotating,ranade2025using,ma2025should,he2024if}. While some have 
 proposed that LLMs can serve as zero-shot annotators in natural language processing (NLP) settings \citep{chae2023large,zhang-etal-2025-efficient}, there is less evidence that they can be useful for complex annotations such as those required by the social sciences \citep{guo2024evaluating,karimi-etal-2021-aeda-easier,bucher2024fine,felkner2024gpt,nasution2024chatgpt,pangakis2025keeping,zamfirescu2023johnny}. 
Furthermore, removing humans from the loop entirely may have negative downstream effects in the social sciences, 
where data annotation serves pedagogical purposes. Our goal is to better support RAs in their work, rather than to replace them. 
%To the best of our knowledge, we are the first to consider how RAs (especially from non-technical fields) 
%may interact with LLMs to jointly label data.
An open  question  we  address
is \textit{how RAs will respond given both access to expert and LLM labels}. 
Our work is a direct response to calls within the ICWSM community to build more human-centered annotation systems for CSS \citep{pangakis2024keeping}
and makes several contributions: 
%Incorporating LLMs into annotation workflows can produce over-reliance, where humans defer to LLMs and ignore their own expertise \citep{raees2025exploring}. 
%Furthermore, it is not clear what kinds of information would best enable RAs to instruct LLMs. 
%Previous work has explored various tools for prompt instruction, however, none of these were designed for the social sciences. 


\begin{itemize}
    \item As a team of (computational) social scientists we design \ourmethode{}, a system which distills the social science annotation process and improves over fully automated state-of-the-art approaches for prompt design. This system incorporates 8 different information features which are designed to answer the questions social scientists pose about label quality. 
    \item We evaluate \ourmethode{} with 60 graduate student participants in the area of sustainability and find that they  use our method to improve their prompt design.  
    \item  We find that embedding domain expertise into \ourmethode{} (expert guidance)    is critical for this task, and caution that future work consider the limitations of human-LLM systems without such guidance. 
\end{itemize}

\ourmethode{} is different than existing methods which primarily draw on technical design expertise or which fully automate the annotation process - our goal is to  distill and enhance the social science annotation process and expertise. Towards this end we recruit student participants who would reasonably be hired as RAs for the task of detecting \climate{} in social media posts\footnote{As we are not recruiting RAs, but students who could be hired as RAs and who are representative 
of the pool of potential RAs, for the remainder of the paper we refer to these potential RAs as the study \subs.}. Central to this work is collaboration between non-technical domain experts and computational social scientists -- throughout the paper we consider non-technical domain experts to be trained social scientists with extensive experience both coding data themselves
and advising RAs to do so.
Here, domain experts are  faculty members in the social sciences. 


Our work produces several important findings for human-centered annotation pipelines for CSS, for example \textbf{we find that}: 
 good instructions are needed  for LLMs to detect \climate{} well, a finding we suspect applies to other nuanced concepts; 
 participants can write good instructions with \ourmethode{};
and participants engage with \ourmethode's information features  and prefer natural language over statistics.
We demonstrate that LLMs can enable data labeling in CSS settings, however, 
we also sound a cautionary note that even human-centered pipelines will likely require domain expertise when the task is to label
difficult concepts.

 
 %While LLMs can improve with fine-tuning in social science settings \citep{alizadeh2025open}, this requires human data and defeats the purpose of using them as zero-shot annotators where they perform the task that a human would. 

\commentout{
Instead of  using LLMs as single zero-shot annotators, a more promising approach may be to develop collaborative human-LLM workflows for data annotation and prompt design \citep{shin2024understanding,li2023coannotating,ranade2025using,ma2025should,he2024if} and to utilize crowds of LLMs instead of single models \citep{zhang-etal-2025-efficient}. However,  incorporating LLMs into annotation workflows can produce over-reliance, where humans defer to LLMs and ignore their own expertise \citep{raees2025exploring}. Thus, a successful method for a social science setting would steer RAs towards social science expertise, over LLM outputs, while still allowing users to learn from and refine their knowledge given useful content from LLMs. }

\commentout{

\begin{itemize}
    \item  Collaborative co-design of \ourmethod{}, a system which distills the social science annotation process and improves over fully automated state-of-the-art approaches for prompt design.
    \item An analysis from two empirical studies about how \subs{} instruct LLMs to detect public attitudes around climate change in social media data.
    \item Research findings which contribute to the study of human-LLM interactions e.g.:  Good instructions are needed  for LLMs to detect \climate{} well; participants can write good instructions with \ourmethod{}, especially with  guidance; Participants engage with \ourmethod's information features  and prefer natural language over statistics.
\end{itemize}



To realize the potential of LLMs in assisting with data annotation, we  develop \ourmethod{} through a collaborative co-design process with social and computer scientists (described in \secref{sec:sys}).
\ourmethode{} is a  collaborative RA-LLM system where RAs can instruct LLMs about how best to annotate data. This generates a set of diverse instructions, each of which can be used to train different LLMs, resulting in a crowd of LLMs which can perform annotation at a scale which surpasses that of RAs as annotators. 
\ourmethode{} is different than existing methods which primarily draw on technical design expertise or which fully automate the annotation process - our goal is to  distill and enhance the social science annotation process and expertise. In order to overcome the known challenge of over-reliance, 
we develop a second  versions of our system, \ourmethode,
which is designed to nudge users towards the judgments of social scientists rather than LLM outputs. 




We evaluate \ourmethod{} through two user studies (the design of which is described in \secref{sec:empdesign}). In both studies \subs{} are charged with the task of instructing LLMs to annotate social media posts for the concept of \textit{\climate{}}
(introduced in \secref{sec:climate})
. 
In the first user study, we instruct RAs around the target task, provide a definition of the target concept, and access to \ourmethod. 
In the second study, \subs{} use \ourmethode{} which includes expert scaffolding (three new instructional components around the target concept designed to nudge \subs{} towards the judgments of social scientists). 
As we are not recruiting RAs, but students who could be hired as RAs and who are representative 
of the pool of potential RAs, for the remainder of the paper we refer to these potential RAs as the study \subs. 
Our empirical work produced the  key findings described under our contributions above (which are also described in \secref{sec:empresults})
and contributes to the related work outlined in \secref{sec:relatedwork}. 

}



% There are many processes in social science annotation - we want to show we know / understand 

==> AnonymousSubmission/LaTeX/new_intro.tex <==


\section{Introduction}
 While some have 
 proposed that large language models (LLMs) can serve as zero-shot annotators in natural language processing (NLP) settings \citep{chae2023large,zhang-etal-2025-efficient}, there is less evidence that they can be useful for complex annotations such as those required by the social sciences \citep{guo2024evaluating,karimi-etal-2021-aeda-easier,bucher2024fine,felkner2024gpt,nasution2024chatgpt,pangakis2025keeping,zamfirescu2023johnny}. 
Instead, there have been calls for human-centered workflows for annotation \citep{shin2024understanding,li2023coannotating,ranade2025using,ma2025should,he2024if}.
Our work responds to these calls with a system, \ourmethode{}, which is designed for computational social science (CSS) research settings.
The goal of \ourmethode{} 
is to support researchers in grounding LLMs in their concept definition, both when that concept definition is still undergoing specification and when it is well-specified. 
%is to assist the data labeling process by allowing researchers to assess the quality and reliability of LLM labels for social media data. %We do this  by supporting both concept specification and LLM alignment.

% Consider the case where a researcher has an idea of a concept
Consider a researcher with an idea of a concept they would like to mine in social media data, such as climate pessimism. Typically, they may explore the data and refine the concept through examples. Next, they may describe this concept to a group of research assistants and iteratively develop a codebook to specify how the concept should be coded. Here, they may still refine the concept through feedback from the labelers. We refer to the first process as \spec, where the concept is defined in increasingly concrete terms. 
We refer to the second process as grounding, where the goal is to align labelers with the new specification.    
We bring together social scientists from diverse fields and computational scientists to design information features for interrogating LLM outputs which support \align{} to both evolving and existing specifications.
These features are designed to mimic key aspects of the social science annotation pipeline, such as evaluating label consistency and reliability, and providing natural language explanations.
%\gs{again, we don't really do this.}

%Our focus is on the setting where we would like to assign labels to social media posts. 

%For example, we determined that label reliability is as important as label quality in communicating about analyses and implemented a set of features for thinking about reliability. 

We  evaluate our system in a setting with high social impact and where we expect LLMs to struggle: the task of detecting pessimism with respect to the ability to mitigate the effects of climate change (\climate). 
The  abundance of negative political content on social media platforms may
 cause users  to feel overwhelmed, anxious, and fatigued with news and politics,  leading to cynicism and lower levels of political efficacy \citep{lane2025worn,hasell2025social,song2021social}.
 Yet, it is an open question how this relates to attitudes towards climate change. 
Like others \citep{galdeman2025mapping,pearce2019social,treen2022discussion,hautea2021showing}, we utilize social media data  as a key source for insights into public attitudes about climate change. 
%One result may be 
%that the public will become increasingly convinced that actions to mitigate the consequences of climate change are futile. 
%We refer to this attitude as \textbf{\climate}. 


We design two studies to evaluate \ourmethode. In the first, we assume that the target concept is not yet specified. This represents the case where specification and grounding may occur simultaneously, such as when a researcher iterates with labelers to develop a codebook. 
In the second, we assume that the concept has been specified. Here, \subs{} have access to a  limited amount of ground-truth labels which they can use to evaluate the LLM. 
In both cases we evaluate the ability of \ourmethode{} to support \align, asking whether \subs{} can improve the ability of LLMs to detect \climate{} through interaction with our system. 
We recruit 60 participants from a graduate program on the environment and 
sustainability to use our system to detect \climate{} in TikTok posts.
%We find that \ourmethode{} is effective in both settings.




%We explore two settings which occur in CSS data annotation workflows.
%\gs{I would try to keep this consistant.  Either different stages or different settings.  Let's not change back and forth willy nilly like now.  I would vote for settings.}
%In the first, the researcher may have a certain concept in mind but not yet have a mature operationalization of that concept. For example, they may not yet know how to define this concept for a codebook, or in a manner which can be easily explained to another or to an LLM. In this case, a researcher can use our system to hone in on different concept operationalizations through experimenting with different instrumentations.
%to explore how an LLM may respond to different operationalizations and instructions, as the researcher explores the concept through the data. \
%gs{I think we want to be more careful with the language about operationalization and instructions.  I feel like here it can help uses to home in on an operationalization by experimenting with different instrumentations.}
%In the second setting, the researcher has a settled conceptualization and access to a limited amount of ground-truth labels which they can use to evaluate the LLM. We find that \ourmethode{} is effective in both settings.


 We present \ourmethode{} as a CSS contribution and evaluate it on a carefully selected case study. 
 %\gs{I don't think we do evaluate it extensively.  We only have one concept, for example.}
 %with human participants. 
 We also introduce the problem of detecting \climate, an important attitude that integrates sustainability, communication, and political science research. We find that while \ourmethode{} is effective for improving LLM outputs, there is still room to improve on the task of detecting \climate. 



==> AnonymousSubmission/LaTeX/results.tex <==
\subsection{Empirical Study Results}
\label{sec:empresults}

Three social science team members annotated a subset of the TikTok videos and the ground truth label was set to be the majority vote across their labels. Experts detected \climate{} in only 10\% of videos in the 10 videos. In contrast, across all prompts and conditions LLMs tended to detect \climate{} in 58.7\% of posts. Thus, the task of producing alignment between the LLM's output and expert labels is particularly difficult for the concept of \climate.


 We generate LLM outputs given the combination of instructions written by \subs{} and a system prompt (shown in the Appendix~\nameref{app:systemPrompt}). 
Each LLM output will contain a ``Yes'' or ``No'' label as to whether the video contains \climate. 
We can then calculate a metric, such as accuracy, given these generated labels and the ground truth labels from the team members. 

For example, to calculate the change in accuracy between initial instructions participants wrote and later instructions  we would do the following. 
First, we obtain the set of ground truth annotations, 
$y$. Then, for each participant, indexed by $j\in J$, we generate a set of annotations  for instructions $0$, $y^0_j$.
Similarly, we can produce a set of annotations for each participant given  later instructions, $k$, $y^k_j$. 
Then to calculate the average change in accuracy between the final and initial instructions we would compute the following: 

$$\frac{1}{|J|}\sum_{j\in J}(Accuracy(y_j^k)-Accuracy(y_j^0)),$$



where the Accuracy is evaluated on the ground truth annotations $y$. 

 


\commentout{
\begin{figure}[ht]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
  \includegraphics[width=\linewidth]{AnonymousSubmission/fig/group_majority_yes_count_lineplot.pdf}
  \caption{\sone: We see that \subs{} who begin by assigning more than 50\% of videos the label ``Yes''
  assign fewer ``Yes'' labels after using \ourmethod{} (100\% to 90\%). This is generally a positive sign, as they are overall assigning far more positive labels than the social science experts who only assign the positive label to 10\% of videos. However, we also see that \subs{}
  who begin by assigning fewer than 50\% of videos the label ``Yes'' actually assign the label more often after using \ourmethod{} (30\% to 40\%). This suggests that they may be influenced by the LLM which tends to assign the positive label often (initially 80\% and then 60\% of the time). 
  }
  \label{fig:majority_yes_count}
  \end{subfigure}
% \end{figure}
    \hfill
% \begin{figure}[ht]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
  \includegraphics[width=\linewidth]{AnonymousSubmission/fig/group_majority_yes_study2.pdf}
  \caption{\stwo: We see that \subs{} who begin by assigning more than 50\% of videos the label ``Yes''
  assign fewer ``Yes'' labels after using \ourmethod{} (70\% to 60\%). This is generally a positive sign, as they are overall assigning far more positive labels than experts who only assign the positive label to 10\% of videos. In \stwo{} we see that \subs{}
  who begin by assigning fewer than 50\% of videos the label ``Yes'' assign the label \textbf{less} often after using \ourmethod{} (10\% to 0\%). In contrast to \sone, here, \subs{} do not seem to be influenced by the LLM which tends to assign the positive label often (70\% to 30\%).  There are several differences between \stwo{} and \sone. The LLM's behavior is directed towards experts more effectively here. Also, on average, \subs{} assign the label far less often than in \sone, in a much clearer alignment with the frequency with which it is assigned by experts.
   }
  \label{fig:majority_yes_count2}
  \end{subfigure}
\caption{Percentage of ``Yes'' labels for different groups. 
  Participants are asked to annotate the videos themselves twice: once before using \ourmethod{} (Before \ourmethod{} in the figure) and once after (After \ourmethod{} in the figure). 
  \label{fig:both}
  }
\end{figure}
}







\paragraph{RQ1: Can \subs{} use \ourmethode{} to improve their instructions to LLMs?}
To answer this we compare the performance between the selected prompt and the first prompt. 
In \tabref{tab:prompt_performance24}, we see that the performance of the prompts provided with instructions written after 
\subs{} used \ourmethode{} is higher than that of the first prompts.  The improvement of the accuracy, precision, and F-Measure are all statistically significant. 


The  length of \subs' instructions also increased substantially over time, with initial instructions averaging 309.2 characters and final instructions averaging 737.8 characters. This lengthening reflects more detailed instructions, richer definitions, and inclusion of edge cases—all of which may have contributed to improved LLM performance. For example, we include P12's full initial and final instructions in Appendix~\nameref{app:p12}, P12's final instructions contain multiple edge cases and provide a decision boundary, with more detail than their first prompt.
% For example, as \tabref{tab:p12_prompts} shows, P12's final instructions contains multiple edge cases and provides a decision boundary, and became a lot more detailed than their initial instructions.

\paragraph{RQ2: When equipped with instructions from \ourmethode{} how do LLMs compare with participants?}
We see in \tabref{tab:prompt_performance24}  that LLMs achieved a similar performance as \subs{}
when supplied with selected instructions. When supplied with the first prompts it is less clear that LLMs can achieve a similar performance as \subs. 
This demonstrates the need for an iterative system whereby \subs{}
can improve their instructions through exposure to information. 


\paragraph{RQ3:  How does \ourmethode{} compare with a state-of-the-art automated method?}
We compare against \emph{Automatic Prompt Engineer (APE)} \citep{ape_zhou2023}. APE treats natural-language instruction as a program and performs black-box optimization: an LLM proposes candidate instructions from input–output demonstrations; the target model scores candidates on a chosen metric; and the system iteratively filters and paraphrases high-scoring prompts before returning the top instruction. 
We run APE on the same tasks and scoring criteria  as our method.

Since generating a good first prompt is challenging, to judge APE fairly, we provide it with the selected instructions and the system prompt for each participant, rather than demanding that it come up with its own prompt from scratch. 
We then average the performance across all 60 selected prompts from the two studies. 



We see in \tabref{tab:prompt_performance24} that \ourmethode{} improves over APE in terms of accuracy, precision, and F-Measure. 
The recall is slightly lower. This is due to the fact that the prompts produced by APE lead to positive labels 72.05\% of the time. 
%Moreover, we see a stronger improvement relative to APE with \ourmethode. 

\input{AnonymousSubmission/LaTeX/big_table}

\begin{figure}
\centering
%\begin{minipage}[t]{0.49\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{AnonymousSubmission/fig/feature_helpfulness_scatter.pdf}
  \captionof{figure}{Participants in \stwo{} were asked to rate the helpfulness of each feature. We see that the features that included natural language tended to be viewed as more helpful than the statistical features.}
  \label{fig:feature_helpfulness_scatter}

\end{figure}

\paragraph{RQ4: Which information features do \subs{} use and do they find the system usable?}
In \figref{fig:feature_co_usage_heatmap} we see which features were selected with which other features. 
In particular, \subs{} tended to use the \annexpl, \anncert, and \statren, features the most. 
In \sone{} we also asked \subs{} to respond to a free-text question asking which features they found most helpful. 
There, we found that \subs{} most frequently mentioned \annexpl. 
In \stwo{} we updated this question so that \subs{} where asked to rate each of the 
information features on a scale from ``not at all helpful'' to ``extremely helpful''. 
Inspecting this data in \figref{fig:feature_helpfulness_scatter}, we see that \subs{} rated \annexpl{} as the most helpful on average, scoring 4.36 on a 1 to 5 scale. 




Overall, participants responded positively to \ourmethode. The average System Usability Scale (SUS) score across all participants was 67, and the median was 68, with the 75 percentile scoring at 75 indicating high perceived usability. According to standard SUS interpretation, scores above 68 are considered above average, and scores above 80 are typically considered excellent. This suggests that the interface effectively supported \subs' workflows despite their limited technical backgrounds.

Specific ratings for each SUS question can be found in \figref{fig:sus_stacked_barplot}. Likert scale ratings in the range of 1-2 are classified as Disagree, 3 is classified as Neutral, and 4-5 are classified as Agree. Most positively worded questions received high agreement. However, the item ``I would use this system frequently'' received a notable number of neutral responses. This may be due to the specific nature of the annotation task, which is primarily relevant for research or specialized data analysis use cases, rather than for tasks that participants would do on a daily basis.




\paragraph{RQ5:  Will \ourmethode{} produce LLM outputs with more alignment with experts than \ourmethode?}
To answer this question we inspect the performance both of \subs{}  and of the instructions they wrote, in each study.  
 In \tabref{tab:prompt_performance24} we see that in \stwo, when provided with expert guidance, \subs{} wrote instructions that performed better than those written without the guidance. This is true across all performance metrics. 
Furthermore, in \sone{} \subs{} agreed with experts on the 10 videos they labeled 52\% of the time on average. In \stwo, they agreed with experts 73\% of the time on average. 
Thus we see that in \stwo{}  \subs{} exhibited better understanding of \climate{} \textit{and}  ability to guide LLMs towards alignment with experts.
 
\begin{figure}

  \centering
  \includegraphics[width=.8\linewidth]{AnonymousSubmission/fig/feature_co_usage_heatmap_triangular.pdf}
  \captionof{figure}{The number of times features were used. By reading the diagonal we can see that most of the 60 \subs{} used all features, with S-Trend being used the most often.}
  \label{fig:feature_co_usage_heatmap}

\end{figure}

\begin{figure*}
  \centering
  \includegraphics[width=.69\linewidth]{AnonymousSubmission/fig/sus_stacked_barplot.pdf}
  \caption{Participants completed the SUS  with respect to \ourmethode.
    We see that overall the system is usable and does not require a technical background. The numbers in the bars refer to the number of participants who selected this option.}
  \label{fig:sus_stacked_barplot}
\end{figure*}


%\input{small_table}


To probe whether this improvement was influenced by the expert components, we asked in the \stwo{} post-survey which resources most helped \subs{} arrive at their definition of \climate. Respondents most often cited using their own knowledge (30.3\%) and the expert-labeled examples shown at the beginning of the study (27.3\%), followed by seeing how experts would label the example data in the \ourmethode{} table (24.2\%), leading to a total of over half of the participants (51.5\%) drawing most from expert-provided information.
A small share of participants selected the general platform information (12.1\%) and the LLM explanations ($\sim$6\%). 
%This suggests that the expert guidance can provide an additional anchor point beyond LLM outputs, leading to higher quality LLM instructions and better alignment with experts.

%This pattern suggests that participants anchored their definitions in examples and expert guidance rather than in the LLM’s explanations, consistent with the higher expert-alignment we observe in \stwo{}.


==> AnonymousSubmission/LaTeX/small_table.tex <==

\begin{table*}[t]
\small
\caption{The performance metrics for each study. 
We inspect both how well the \subs{} perform when annotating the data themselves,
and how well the LLMS perform on their selected prompts. 
} 
\label{tab:prompt_performance}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
 & Labels produced by & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F-Measure} & \textbf{Average  Length of Instructions}\\
\midrule
\sone & Participants & $0.522_{0.039}$ & $0.167_{0.040}$ & $0.667_{0.093}$ & $0.247_{0.046}$ & -\\
\sone & Final prompt & $0.514_{0.008}$ & $0.214_{0.015}$ & $0.901_{0.040}$ & $0.318_{0.019}$ & 632.3\\

\midrule
\stwo & Participants & $0.730_{0.033}$ & $0.154_{0.038}$ & $0.485_{0.088}$ & $0.219_{0.047}$ & -\\
\stwo& Favorite prompt&$0.631_{0.006}$ & $0.272_{0.012}$ & $0.939_{0.000}$ & $0.400_{0.010}$ & 843.3\\
\stwo & Final prompt & $0.629_{0.010}$ & $0.380_{0.024}$ & $0.502_{0.019}$ & $0.375_{0.015}$ & 867.7\\

\midrule
\end{tabular*}
\end{table*}


==> AnonymousSubmission/LaTeX/temp.tex <==
In the two studies we address the following research questions: 

\begin{itemize}
    \item \textbf{RQ1:} How do the outputs produced with instructions that \subs{} construct with \ourmethode{} compare with those produced with the system prompts written with minimal intervention?
    \item \textbf{RQ2:} How do the outputs produced with instructions that \subs{} construct with \ourmethode{} compare with those produced with the system prompts written with automated methods for intervention?
    \item \textbf{R3:} Can \subs{} use \ourmethode{} to improve their instructions to LLMs?
   \item  \textbf{RQ4:} Which information features do \subs{} use and do they find the system usable overall?
\end{itemize}




To answer the first four research questions we utilize a set of ground truth annotations for 10 TikTok videos.
Each video is annotated by the team members and we take the majority vote to arrive at a single ground truth label 
of ``Yes'' - the video contains \climate, or ``No'' - it doesn't. 
As we saw in \secref{sec:so}, we generate LLM outputs given the combination of instructions written by \subs{} and a system prompt. 
Each LLM output will contain a ``Yes'' or ``No'' decision label as to whether the video contains \climate. 
We can then calculate a metric, such as accuracy, given these generated labels and the ground truth labels from the team members. 

For example, to calculate the change in accuracy between initial instructions participants wrote and later instructions in \sone{} we would do the following. 
First, we obtain the set of ground truth annotations, 
$y$. Then, for each participant, indexed by $j\in J$, we generate a set of annotations  for instructions $0$, $y^0_j$.
Similarly, we can produce a set of annotations for each participant given  later instructions, $k$, $y^k_j$. 
Then to calculate the average change in accuracy between the final and initial instructions for study one we would compute the following: 

$$\frac{1}{|J|}\sum_{j\in J}(Accuracy(y_j^k)-Accuracy(y_j^0)),$$



where the Accuracy is evaluated on the ground truth annotations $y$.

